Constructive Interpretability with CoLabel: Corroborative Integration, Complementary Features, and Collaborative Learning

Machine learning models with explainable predictions are increasingly sought after, especially for real-world, mission-critical applications that require bias detection and risk mitigation. Inherent interpretability, where a model is designed from the ground-up for interpretability, provides intuitive insights and transparent explanations on model prediction and performance. In this paper, we present CoLabel, an approach to build interpretable models with explanations rooted in the ground truth. We demonstrate CoLabel in a vehicle feature extraction application in the context of vehicle make-model recognition (VMMR). CoLabel performs VMMR with a composite of interpretable features such as vehicle color, type, and make, all based on interpretable annotations of the ground truth labels. First, CoLabel performs corroborative integration to join multiple datasets that each have a subset of desired annotations of color, type, and make. Then, CoLabel uses decomposable branches to extract complementary features corresponding to desired annotations. Finally, CoLabel fuses them together for final predictions. During feature fusion, CoLabel harmonizes complementary branches so that VMMR features are compatible with each other and can be projected to the same semantic space for classification. With inherent interpretability, CoLabel achieves superior performance to the state-of-the-art black-box models, with accuracy of 0.98, 0.95, and 0.94 on CompCars, Cars196, and BoxCars116K, respectively. CoLabel provides intuitive explanations due to constructive interpretability, and subsequently achieves high accuracy and usability in mission-critical situations.

==> Makefile <==
# Makefile for LaTeX files

PACKAGE=acmart

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
PANDOC = pandoc

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

PDFPICS :=
#PDFPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.pdf$$/) { print "$$foo[2] "; } else { print "$$foo[2].pdf "; }}' *.tex)
DEP	= *.tex

TRG	= $(SRC:%.tex=%.pdf)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

all 	: $(TRG)

define run-latex
	  $(COPY);$(LATEX) $<
	  egrep -q $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	  $(RM) $(<:%.tex=%.toc.bak)
	  # Display relevant warnings
	  egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

$(TRG)	: %.pdf : %.tex $(DEP) $(PDFPICS) $(BIBFILE)
	  @$(run-latex)

.PHONY	: all show clean ps pdf showps text stylecheck spellcheck

view:
	acroread $(PDF)

osx:
	open $(PDF)

text: *.tex
	$(PANDOC) --wrap=none -s $< -o $@

doc: *.tex
	$(PANDOC) --wrap=none -s $< -o $@

combined:
	pdfunite response.pdf logging.pdf combined.pdf

# Check style:
stylecheck:
	printf "weasel words: "
	sh ./scripts/weasel *.tex
	printf "\npassive voice: "
	sh ./scripts/passive *.tex
	printf "\nduplicates: "
	perl ./scripts/dups *.tex
	printf "\ndone\n"

# Check spelling with aspell
spellcheck:
	find . -name "*.tex" -exec aspell --lang=en --mode=tex --dont-suggest --personal=./.aspell.en.pws check "{}" \;

######################################################################
# Define rules for PDF source files.
%.pdf: %.eps
	epstopdf $< > $(<:%.eps=%.pdf)


docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.bak

distclean: docclean
	$(RM)  *.pdf 

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.pdf=%.aux) $(TRG:%.pdf=%.bbl) $(TRG:%.pdf=%.blg) $(TRG:%.pdf=%.log) $(TRG:%.pdf=%.out)

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'
